Clustering under Perturbation Stability in Near-Linear Time

We consider the problem of center-based clustering in low-dimensional Euclidean spaces under the perturbation stability assumption. An instance is $\alpha$-stable if the underlying optimal clustering continues to remain optimal even when all pairwise distances are arbitrarily perturbed by a factor of at most $\alpha$. Our main contribution is in presenting efficient exact algorithms for $\alpha$-stable clustering instances whose running times depend near-linearly on the size of the data set when $\alpha \ge 2 + \sqrt{3}$. For $k$-center and $k$-means problems, our algorithms also achieve polynomial dependence on the number of clusters, $k$, when $\alpha \geq 2 + \sqrt{3} + \epsilon$ for any constant $\epsilon > 0$ in any fixed dimension. For $k$-median, our algorithms have polynomial dependence on $k$ for $\alpha > 5$ in any fixed dimension; and for $\alpha \geq 2 + \sqrt{3}$ in two dimensions. Our algorithms are simple, and only require applying techniques such as local search or dynamic programming to a suitably modified metric space, combined with careful choice of data structures.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We presented near-linear time algorithms for finding optimal solutions of stable clustering instances for the $k$-means, $k$-medians, and $k$-center problem.
Our algorithms are simple and fast, making them practical for large datasets.

It would be interesting to see whether these approaches could be extended to other metric spaces, such as those with bounded doubling dimension.
It would also be interesting to extend our approaches to work for stable instances with a smaller values of $\alpha$.

